A priori convergence estimates for a rough Poisson-Dirichlet problem with natural vertical boundary conditions

Stents are medical devices designed to modify blood flow in aneurysm sacs, in order to prevent their rupture. Some of them can be considered as a locally periodic rough boundary. In order to approximate blood flow in arteries and vessels of the cardio-vascular system containing stents, we use multi-scale techniques to construct boundary layers and wall laws. Simplifying the flow we turn to consider a 2-dimensional Poisson problem that conserves essential features related to the rough boundary. Then, we investigate convergence of boundary layer approximations and the corresponding wall laws in the case of Neumann type boundary conditions at the inlet and outlet parts of the domain. The difficulty comes from the fact that correctors, for the boundary layers near the rough surface, may introduce error terms on the other portions of the boundary. In order to correct these spurious oscillations, we introduce a vertical boundary layer. Trough a careful study of its behavior, we prove rigorously decay estimates. We then construct complete boundary layers that respect the macroscopic boundary conditions. We also derive error estimates in terms of the roughness size epsilon either for the full boundary layer approximation and for the corresponding averaged wall law.

==> PreuveKondrjavcev.tex <==
\begin{proof}
We make a change of variables $x_1=r\cos \vartheta,x_2=r \sin \vartheta,\vartheta =0 $, leading to rewrite $I$ as
$$
I=\int_0^\infty \int_0^\infty \frac{\left|\xi(\rho+h,0)-\xi(\rho ,0)\right|^2}{h^{2-\alpha}} \, d\rho  \, dh ,
$$
note that the second space variable for $\xi$ is now $\vartheta = 0$.
We insert terms inside the domain, namely
$$
\begin{aligned}
I & \leq \int\int_0^\infty \frac{ \left| \xi (\rho+h,0) - \xi \left(\rho+h,\atan\frac{h}{\rho}\right) \right|^2}{h^{2-\alpha}} +\frac{ \left| \xi \left(\rho+h,\atan\frac{h}{\rho}\right) - \xi \left(\rho,\atan\frac{h}{\rho}\right) \right|^2}{h^{2-\alpha}}  d\rho  \, dh  \\
& + \int_0^\infty \int_0^\infty \frac{ \left| \xi \left(\rho,\atan\frac{h}{\rho}\right) - \xi \left(\rho,0\right) \right|^2}{h^{2-\alpha}}  d\rho  \, dh =: I_1 + I_2 + I_1' \\
\end{aligned}
$$
Obviously the terms $I_1$ and $I_1'$ are treated the same way. We make a change of variable $(\rho,h=\rho \tan \vartheta )$ 
$$
I_1 = \int_0^{\frac{\pi}{2}} \int_0^\infty \frac{ \left| \xi (\rho(1+\tan \vartheta),0) - \xi (\rho(1+\tan\vartheta),\vartheta  ) \right|^2}{(\rho \tan \vartheta )^{2-\alpha}}\frac{\rho}{1+\vartheta^2}  d\rho  \, d\vartheta   \\
$$
in order to eliminate the dependence on $\vartheta$ in the first variable of $\xi$ we make the change of variable
$(\rho=r/(1+\tan\vartheta),\vartheta)$ which gives
$$
I_1 = \int_0^{\frac{\pi}{2}}\int_0^\infty  \frac{ \left| \xi (r,0) - \xi (r,\vartheta  ) \right|^2}{r^{2-\alpha}} r dr  \frac{(1+\tan\vartheta)^{\alpha}}{\tan^{2-\alpha} \vartheta (1 + \vartheta^2) } \,d\vartheta 
\leq  \int_0^\infty \int_0^{\frac{\pi}{2}} \frac{ \left| \xi (r,0) - \xi (r,\vartheta  ) \right|^2}{r^{2-\alpha}} r dr \,\frac{d\vartheta}{\vartheta^{2-\alpha}}
$$
We are in the hypotheses of the Hardy inequality thus we have
$$
I_1 \leq \frac{4}{(1-\alpha)^2} \int_0^\infty  \int_0^{\frac{\pi}{2}} \left| \dd{\xi}{\vartheta }(r,\vartheta)  \right|^2 \vartheta^{\alpha}d\vartheta  r^{\alpha -1} dr \leq K  \int_0^\infty  r^\alpha \int_0^{\frac{\pi}{2}} \frac{1}{r^2} \left| \dd{\xi}{\vartheta }(r,\vartheta)  \right|^2 d\vartheta r dr \leq \nrm{\xi}{\alpha}^2   
$$
In the same manner
$$
\begin{aligned}
I_2 & \leq   \int_0^{\frac{\pi}{2}} \int_0^\infty \frac{ \left| \xi (\rho(1+\tan \vartheta),\vartheta ) - \xi (\rho,\vartheta  ) \right|^2}{(\rho \tan \vartheta )^{2-\alpha}}\rho  d\rho  \, d\vartheta \\
& =  \int_0^{\frac{\pi}{2}} \int_0^\infty \left| \int_0^{\rho \tan \theta } \dd{\xi}{\rho} ( \rho + s ,\vartheta ) ds \right|^2 \rho^{\alpha-1}  d\rho   \frac{d \vartheta }{\tan^{2-\alpha}\vartheta }\\
& \leq \int_0^{\frac{\pi}{2}} \left\{ \int_0^{\tan \vartheta } \left[  \int_0^\infty  \left| \dd{\xi}{\rho} \right|^2 ( \rho(1 + \sigma ) ,\vartheta ) \rho^{ 1+\alpha} d\rho \right]^\ud d \sigma \right\}^2  \frac{d \vartheta }{\tan^{2-\alpha}\vartheta  }
\end{aligned}
$$
where we made the chage of variables $s=\rho\sigma$ and applied the generalized Minkowski inequality. Now we set
$r=\rho(1+\sigma)$ inside the most interior integral above
$$
I_2\leq  \int_0^{\frac{\pi}{2}} \left\{ \int_0^{\tan \vartheta }\frac{d\sigma }{(1+\sigma)^{1+\frac{\alpha}{2}}}  \left[  \int_0^\infty  \left| \dd{\xi}{\rho} \right|^2 (r,\vartheta) r^{1+\alpha} dr\right]^\ud \right\}^2  \frac{d \vartheta }{\tan^{2-\alpha} \vartheta } 
$$
Now, we have  separated the integrals in $\sigma$ and $r$, the part depending on $\sigma$  is easy to integrate.
Thus we obtain
$$
I_2 \leq \int_0^{\frac{\pi}{2}} {\cal S}(\vartheta)   \int_0^\infty  \left| \dd{\xi}{\rho} \right|^2 (r,\vartheta) r^{1+\alpha} dr  d\vartheta ,\text{ where }  {\cal S}(\vartheta)= \frac{1}{\tan^{2-\alpha}\vartheta }  \left[ \frac{1}{(1+\tan \vartheta )^{\frac{\alpha}{2}}} -1 \right]^2 
$$ 
Distinguishing whether $\tan \vartheta$ is greater or not than 1, it is possible to show that ${\cal S}$ is uniformely bounded wrt $\vartheta$ which gives
again the desired result.
\end{proof}


%$$
% \int_0^{\tan \vartheta }\frac{d\sigma }{(1+\sigma)^{2+\alpha}} = K(\alpha) \left[ \frac{1}{(1+\sigma)^{\frac{\alpha}{2}} \right]^{\tan \sigma}_0
%$$

